NTIRE 2025 the 2nd Restore Any Image Model (RAIM) in the Wild Challenge

In this paper, we present a comprehensive overview of the NTIRE 2025 challenge on the 2nd Restore Any Image Model (RAIM) in the Wild. This challenge established a new benchmark for real-world image restoration, featuring diverse scenarios with and without reference ground truth. Participants were tasked with restoring real-captured images suffering from complex and unknown degradations, where both perceptual quality and fidelity were critically evaluated. The challenge comprised two tracks: (1) the low-light joint denoising and demosaicing (JDD) task, and (2) the image detail enhancement/generation task. Each track included two sub-tasks. The first sub-task involved paired data with available ground truth, enabling quantitative evaluation. The second sub-task dealt with real-world yet unpaired images, emphasizing restoration efficiency and subjective quality assessed through a comprehensive user study. In total, the challenge attracted nearly 300 registrations, with 51 teams submitting more than 600 results. The top-performing methods advanced the state of the art in image restoration and received unanimous recognition from all 20+ expert judges. The datasets used in Track 1 and Track 2 are available at https://drive.google.com/drive/folders/1Mgqve-yNcE26IIieI8lMIf-25VvZRs_J and https://drive.google.com/drive/folders/1UB7nnzLwqDZOwDmD9aT8J0KVg2ag4Qae, respectively. The official challenge pages for Track 1 and Track 2 can be found at https://codalab.lisn.upsaclay.fr/competitions/21334#learn_the_details and https://codalab.lisn.upsaclay.fr/competitions/21623#learn_the_details.

==> sec/2_challenge.tex <==
\section{NTIRE 2025 the 2nd RAIM Challenge}
\label{sec:challenge}

\subsection{Training Data}
In this challenge, participants can train their models using any data they can collect and any pre-trained models they can access, as in the 1st RAIM.

\subsection{Validation and Test Data}

To facilitate the design and development of RAIM by participants, we provide two types of validation and test data: paired data with reference ground-truth (R-GT), and unpaired data.


\subsubsection{Paired Data with R-GT}
% To facilitate the model validation, we first provide some paired data in the following scenarios, where both the input low-quality image and the high-quality R-GT can be collected. Examples can be found in Figure~\ref{data1}.

\begin{figure*}
  \centering
  \includegraphics[width=1\textwidth]{fig_track1_2025/pa.jpg} 
  \caption{Example Paired data for each track we have provided.} 
  \label{data_pair} 
  \vspace{2em}
\end{figure*}

\begin{figure*}
  \centering
  \includegraphics[width=1\textwidth]{fig_track1_2025/un.jpg} 
  \caption{Example Unpaired data for each track we have provided.} 
  \label{data1_unpair} 
  \vspace{2em}
\end{figure*}

To facilitate the model validation, we first provide some paired data in the following scenarios, where the R-GTs are of high quality and the input images are constructed via the real calibrated parameters and are processed via the real camera image signal processor (ISP).

In specific, in track one, \ie, the low-light joint denoising and demosaicing (JDD) task, we first calibrate the noise distribution of the camera sensor and the point spread function (PSF) of the camera lens, and then simulate the input raw images by applying the noise and the PSF in different intensities. In this way, we can get the paired data with both a high-quality R-GT (captured by a high-end DSLR) and a low-quality input that is as close to the real inputs as possible. For participants unacquainted with the raw-related tasks, we also provide the basic raw image processing codes for reference. We select sensors and lenses that are commonly applied in recent flagship smartphones (whose test data are also provided in phase 1 and phase 3), and the calibration of noise and the approximate PSF is also given for participants to simulate the training data. All data in track one can be available now at \url{https://drive.google.com/drive/folders/1Mgqve-yNcE26IIieI8lMIf-25VvZRs_J}.

In track two, \ie, the image detail enhancement/generation task, we first simulate the input raw images as in track one. Then, we process the raw inputs by applying a specific JDD model and a real camera ISP, which conducts tone mapping operations. The JDD model and the tone mapping operations that are key to this pipeline are from the real camera ISP operating in the real flagship smartphones. All data in track two can be available now at \url{https://drive.google.com/drive/folders/1UB7nnzLwqDZOwDmD9aT8J0KVg2ag4Qae}. Examples of two tracks can be found in Fig.~\ref{data_pair}.

We use these data to calculate the full-reference metrics to partially measure the effectiveness of the algorithms and screen the top performers in the early stage.

\subsubsection{Data without R-GT}
In many practical scenarios, the R-GT is very difficult to collect, and the image restoration performance is hard, if impossible, to be measured by full-reference metrics. In this challenge, we provide the data with the following commonly encountered issues in practice.

In track one, we provide raw inputs captured by real camera sensors in a single frame, without any postprocessing and keeping the original noise distribution. The test data covers various scenes (portrait/non-portrait, indoor/outdoor, and so on) and light conditions (different ISO and shutter). More attention should be paid to the following two problems in this track:

\noindent\textbf{Smoothed details and textures}. Limited by hardware and on-chip computing power, images captured by smartphone cameras often face a trade-off between noise/artifact reduction and details/texture richness, impacting the visual quality. The participants are encouraged to keep as rich high-frequency details as possible, to avoid over-smoothed results.

\noindent\textbf{Low-frequency color noise/blocks/bandings}. The low SNR of the input in mobile phone cameras demands a heavy denoising algorithm to output a clean image. However, due to factors such as computing power and storage, the bit-width of the ISP system is limited. When transitioning from the linear domain to the nonlinear domain, visual color noise, blocks, and bandings often appear.


In track two, we provide sRGB images that are captured by real flagship smartphones (the same as the one that provides the paired data). As in track one, the test data cover various scenes (portrait/non-portrait, indoor/outdoor, text, different distances, and so on) and light conditions (different ISO and shutter). More attention should be paid to the following two problems in this track:

\noindent\textbf{Realistic high-frequency detail enhancement or generation}. Limited by camera sensors and on-chip computing power, images captured by smartphone cameras always lack high-frequency details. The participants are encouraged to enhance or generate realistic details to further improve the quality of the image.

\noindent\textbf{Texture adhesion in super-resolution}. In the telephoto mode (e.g., equivalent focal length larger than 230mm), shooting small structures from a distance is an important yet highly challenging task. Texture adhesion greatly deteriorate the user experience.

Examples of two tracks can be found in Fig.~\ref{data1_unpair}.

% \begin{figure*}
%   \centering
%   \includegraphics[width=1\textwidth]{fig/jpgs/data_unpaired.jpg} 
%   \caption{Example input images we have provided without R-GT.} 
%   \label{data2} 
% \end{figure*}

\subsection{Evaluation Measures}

We evaluate the effectiveness of the models with both quantitative measures and subjective evaluation. We also consider the efficiency of the models, including the number of parameters, the FLOPs, and the running time. 

\subsubsection{Quantitative Measure}
\label{quantitativemeasure}

Following prior arts and the 1st RAIM, we employ the PSNR, SSIM, LPIPS, DISTS, and NIQE measures to evaluate the models quantitatively by using the data with R-GT. The evaluation score is computed as follows\footnote{The script of this measure is available at \url{https://sbox.myoas.com/outpublish.html?code=A51c91a521084c0b0#view}.}:

\noindent $SCORE = 20\times \frac{PSNR}{50}+15\times \frac{SSIM-0.5}{0.5}+20\times (1-\frac{LPIPS}{0.4})+40\times (1-\frac{DISTS}{0.3})+30\times (1-\frac{NIQE}{10})$.



\subsubsection{Subjective Evaluation}
\label{qualitativemeasure}

For the test data without R-GT, we judge the perceptual quality of the restored results by visual inspection. Specifically, we invite 10 experienced practitioners and conduct comprehensive user studies for each track. The following features should be considered in the evaluation:

\noindent\textbf{Textures and details}. The restored image should have fine and natural textures and details.

\noindent\textbf{Noise}. Noise, especially color noise, should be eliminated. Some luminance noise should be kept to avoid over-smoothness in flat areas.

\noindent\textbf{Artifacts}. Various artifacts, such as worm-like artifacts, color blocks, bandings, over-sharpening, and so on, should be reduced as much as possible.

\noindent\textbf{Fidelity}. The restored image should be loyal to the given input.

 More details have been discussed during the competition with all participants by referencing specific images and model outputs.

\subsubsection{Efficiency}
\label{efficiency}
In Phase 2 and Phase 3, we consider the efficiency of the model as an important evaluation metric. 
To ensure objectivity and comparability in efficiency evaluation, we establish a standardized efficiency scoring system based on three key factors: parameter count, computational complexity, and inference time.

\noindent\textbf{Parameter Count}. The total number of parameters in the model, measured in millions (M).

\noindent\textbf{Computational Complexity (FLOPs)}. The number of floating-point operations required for a single forward pass on a $1024 \times 1024$ input image, measured in billions (B). 
% If the model cannot process $1024 \times 1024$ inputs due to memory limitations, the input size should be reduced to $512 \times 512$ or, if necessary, $256 \times 256$. The FLOPs are then linearly scaled to the $1024 \times 1024$ equivalent based on pixel ratio.
% For example, if the model runs on $512 \times 512$ input, the measured FLOPs are multiplied by $(1024 \times 1024)/(512 \times 512) = 4$.

\noindent\textbf{Inference Time}. The average forward-pass time per image (in milliseconds) when running the full test set on the same hardware.
% We collect the models of the effective submissions and return the running time of the model to the participants. This calculation is conducted on the same hardware. The outstanding methods in the final phase can also be quantized to run on our hardware platform and get feedback.

For each of the three efficiency metrics—parameter count, FLOPs, and inference time—models are ranked in ascending order, where a lower value indicates better performance. A maximum of 10 points is assigned to the top-ranked model, and the remaining models receive proportionally worse scores based on their rank. The score interval between ranks is calculated as $10/(N-1)$, where 
$N$ is the total number of submitted models. Models with identical metric values share the same score, and subsequent ranks are skipped accordingly to maintain fairness. The final efficiency score is the sum of the scores from three metrics.

\subsection{Phases}

\subsubsection{Phase 1: Model Design and Tuning}
In this phase, participants can analyze the given data and tune their models accordingly. We provided:

\begin{itemize}
\item 50 pairs of paired data in high resolution (i.e., input with reference ground-truth (R-GT)), which can be used to tune the models based on the quantitative measures;

\item 50 images without R-GT, which can be used to tune the model according to visual perception.
\end{itemize}

\subsubsection{Phase 2: Online Feedback}
In this phase, participants can upload their results and get official feedback. We provide:

\begin{itemize}
\item The input low-quality images of another 100 pairs of paired data. 
\end{itemize}

\noindent Only the low-quality input images are provided, and the participants can upload the restoration results to the server and get the quantitative scores online. Users can also upload their results of the images without R-GT provided in Phase 1 to seek feedback. The organizers will provide feedback to a couple of teams that get the highest quantitative scores for the images with R-GT.

\subsubsection{Phase 3: Final Evaluation}
In this phase, we provide the following files for each track:

\begin{itemize}
\item Another 50 images without R-GT for subjective evaluation.
\end{itemize}

\noindent We select the top ten teams according to the quantitative score of the 100 images with R-GT in Phase 2 for each track, and then arrange a comprehensive user study on their results on the above 50 images without R-GT. The final ranks of the ten teams will be decided based on the quantitative scores in phase 2, the efficiency of the model (including \#Parameters, FLOPs, and Running Time of the final model), and the subjective user study results (the weight will be given before the beginning of phase 3).

\subsection{Awards}

The following awards of each track are provided \textbf{for each track}:

\begin{itemize}
\item One first-class award (i.e., the champion) with a cash prize of \textbf{US\$1000};

\item Two second-class awards with cash prizes of \textbf{US\$500 each};

\item Three third-class awards with cash prizes of \textbf{US\$200 each}.
\end{itemize}

\subsection{Important Dates}

\begin{itemize}
\item 2025.02.07: Released data of phase 1. Phase 1 began;
\item 2025.02.24: Released data of phase 2. Phase 2 began;
\item 2025.03.14: Released data of phase 3. Phase 3 began;
\item 2025.03.28: Phase 3 results submission deadline;
\item 2025.04.03: Final rank announced.
\end{itemize}
